Probing a Set of Trajectories to Maximize Captured Information

We study a trajectory analysis problem we call the Trajectory Capture Problem (TCP), in which, for a given input set ${\cal T}$ of trajectories in the plane, and an integer $k\geq 2$, we seek to compute a set of $k$ points (``portals'') to maximize the total weight of all subtrajectories of ${\cal T}$ between pairs of portals. This problem naturally arises in trajectory analysis and summarization. We show that the TCP is NP-hard (even in very special cases) and give some first approximation results. Our main focus is on attacking the TCP with practical algorithm-engineering approaches, including integer linear programming (to solve instances to provable optimality) and local search methods. We study the integrality gap arising from such approaches. We analyze our methods on different classes of data, including benchmark instances that we generate. Our goal is to understand the best performing heuristics, based on both solution time and solution quality. We demonstrate that we are able to compute provably optimal solutions for real-world instances.

==> Makefile <==
# This is the magic latex makefile composed by Dominik Krupke (krupke@ibr.cs.tu-bs.de) for writing papers.
# You can find the corresponding repository at https://gitlab.ibr.cs.tu-bs.de/krupke/magic-latex
# A lot of the ideas are taken and composed from various sources. So feel free to steal it yourself.
-include Makefile.local

# The following variable usually don't need to be altered
TEXFILES:=$(sort $(wildcard *.tex) $(wildcard **/*.tex))

pdf: figures $(TEXFILES)
	latexmk --output-directory=.auxiliary-latex -pdf $(MAIN).tex
	cp ./.auxiliary-latex/$(MAIN).pdf ./$(MAIN).pdf

.DEFAULT_GOAL = all
.PHONY: all check clean

all: pdf

setup: python3
	python3 ./makefile_utils.py --setup

update:
	$(if $(shell command -v wget 2> /dev/null),,$(error Please install `wget` to continue. This should be possible with nearly all package managers. On OS X with Homebrew for example via `brew install wget`))
	wget https://gitlab.ibr.cs.tu-bs.de/krupke/magic-latex/raw/master/Makefile -O Makefile
	wget https://gitlab.ibr.cs.tu-bs.de/krupke/magic-latex/raw/master/makefile_utils.py -O makefile_utils.py

python3:
	$(if $(shell command -v python3 2> /dev/null),,$(error Please install `python3` to continue. This should be possible with nearly all package managers. On OS X with Homebrew for example via `brew install python`))

figures: python3
	python3 ./makefile_utils.py --svg
	python3 ./makefile_utils.py --ipe

autofix: python3
	python3 ./makefile_utils.py --autofix

check: packagecheck spellcheck grammarcheck phrasingcheck fontcheck texcheck

phrasingcheck: python3
	python3 ./makefile_utils.py --diction

packagecheck: python3
	python3 ./makefile_utils.py --packages

fontcheck: python3
	python3 ./makefile_utils.py --fonts

spellcheck:
	python3 ./makefile_utils.py --spell

grammarcheck: python3
	python3 ./makefile_utils.py --grammar

texcheck:
	python3 ./makefile_utils.py --texlint

reference:
	python3 ./makefile_utils.py --saverevision

clean:
	rm -f $(MAIN).pdf
	rm -rf .auxiliary-latex

showchanges:
ifeq ($(VCS),git)
	for texfile in $(TEXFILES); do \
		echo $$texfile; \
		$(VCS) --no-pager diff --color-words $$texfile;\
		done
endif
ifeq ($(VCS),svn)
	for texfile in $(TEXFILES); do \
		echo $$texfile; \
		$(VCS) diff $$texfile; \
		done
endif

diff-pdf:
	latexdiff-vc --$(VCS) --flatten -r $(REFERENCE_REVISION) $(MAIN).tex
	latexmk --output-directory=.auxiliary-latex-diff -pdf $(MAIN)-diff$(REFERENCE_REVISION).tex
	cp ./.auxiliary-latex-diff/$(MAIN)-diff$(REFERENCE_REVISION).pdf .
	rm $(MAIN)-diff$(REFERENCE_REVISION).tex


